Pseudospectral Shattering, the Sign Function, and Diagonalization in Nearly Matrix Multiplication Time

We exhibit a randomized algorithm which given a matrix $A\in \mathbb{C}^{n\times n}$ with $\|A\|\le 1$ and $\delta>0$, computes with high probability an invertible $V$ and diagonal $D$ such that $\|A-VDV^{-1}\|\le \delta$ using $O(T_{MM}(n)\log^2(n/\delta))$ arithmetic operations, in finite arithmetic with $O(\log^4(n/\delta)\log n)$ bits of precision. Here $T_{MM}(n)$ is the number of arithmetic operations required to multiply two $n\times n$ complex matrices numerically stably, known to satisfy $T_{MM}(n)=O(n^{\omega+\eta})$ for every $\eta>0$ where $\omega$ is the exponent of matrix multiplication (Demmel et al., Numer. Math., 2007). Our result significantly improves the previously best known provable running times of $O(n^{10}/\delta^2)$ arithmetic operations for diagonalization of general matrices (Armentano et al., J. Eur. Math. Soc., 2018), and (with regards to the dependence on $n$) $O(n^3)$ arithmetic operations for Hermitian matrices (Dekker and Traub, Lin. Alg. Appl., 1971). It is the first algorithm to achieve nearly matrix multiplication time for diagonalization in any model of computation (real arithmetic, rational arithmetic, or finite arithmetic), thereby matching the complexity of other dense linear algebra operations such as inversion and $QR$ factorization up to polylogarithmic factors. The proof rests on two new ingredients. (1) We show that adding a small complex Gaussian perturbation to any matrix splits its pseudospectrum into $n$ small well-separated components. In particular, this implies that the eigenvalues of the perturbed matrix have a large minimum gap, a property of independent interest in random matrix theory. (2) We give a rigorous analysis of Roberts' Newton iteration method (Roberts, Int. J. Control, 1980) for computing the sign function of a matrix in finite arithmetic, itself an open problem in numerical analysis since at least 1986.

==> Content/inverse.tex <==


\section{Explicit cost and error bounds for triangular matrix inversion}

From \cite{demmel2007fast} we have the cost recurrence
\[C(n) = 2 C(n/2) + 4MM(n/2) + n^2/2 = O(MM(n))\]
assuming $MM(n) = \Theta(n^\gamma)$ for some $2 < \gamma \le 3$. Let us calculate the implied constant in the bound $O(MM(n))$ above. 

By induction suppose that $C(n) \le A * MM(n)$.  Then 
\[ C(n) \le 2 A MM(n/2) + 4 MM(n/2) + n^2/2 \le \]

\subsection{Error analysis}

As in \cite{demmel2007fast}, the starting point of our error analysis is an assumption on the stability of matrix multiplication.  We assume the existence of a matrix multiplication algorithm $Alg$ with the following properties:

\begin{enumerate}
    \item Cost:  The number of arithmetic operations use to multiply two $n \times n$ matrices using $Alg$ is $MM(n) = O(n^\gamma)$ for some $2 < \gamma \le 3$.
    
    \item Stability: If $C = A \cdot B$ is computed using $Alg$, with the computed result $\tilde{C}$, then \[ \Vert \tilde{C} - C \Vert \le \mu(n) \mach_{mach} \Vert A \Vert \Vert B \Vert + O(\mach_{mach}^2)\]
    where $\mu(n)$ is bounded by some low-degree polynomial in $n$.
\end{enumerate}

For example, we may take $Alg$ to be Strassen's algorithm, for which we have $\gamma = 2.81$ and $\mu(n) = n (6n^{\log_2 12} - 5n) = O(n^{4.59})$ \cite{higham1990exploiting}.

We repeat the analysis of triangular matrix inversion in \cite{demmel2007fast} with an eye towards obtaining explicit quantitative error bounds (i.e, replacing big-$O$ notation with an explicit multiplicative constant, and explicitly bounding second-order terms.)

Suppose we wish to compute $C = A \cdot B$ where $A$ and $B$ are only available to us as $\tilde{A}, \tilde{B}$ which have some error.  To be precise, in exact arithmetic we have $C = A \cdot B$, but in reality we have $\tilde{C} = Alg(\tilde{A}, \tilde{B})$, where $\Vert A - \tilde{A} \Vert \le \err(A, n)$ and $\Vert B - \tilde{B} \Vert \le \err(B, n)$.  Then
\begin{align*}\Vert C- \tilde{C} \Vert &\le \Vert \tilde{C} - \tilde{A} \cdot \tilde{B} \Vert + \Vert \tilde{A} \cdot \tilde{B} - C \Vert. 
%&\le \mu(n) \mach \Vert \tilde{A} \Vert \Vert \tilde{B} \Vert +  
\end{align*} 
We know $\Vert \tilde C - \tilde{A} \cdot \tilde{B} \Vert \le \mu(n) \mach \Vert \tilde{A} \Vert \Vert \tilde{B} \Vert$.  Also, we have 
\[  \Vert \tilde{A} \cdot \tilde{B} - C \Vert = \Vert \tilde{A} \tilde{B} - AB \Vert \le \Vert  A \Vert \cdot \err(B,n) + \err(A, n) \cdot \Vert  B \Vert + \err(A, n) \err(B, n).\]
Thus,
\[ \err(C, n) \le \mu(n) \mach \Vert \tilde{A} \Vert \Vert \tilde{B} \Vert + \Vert  A \Vert \cdot \err(B,n) + \err(A, n) \cdot \Vert  B \Vert + \err(A, n) \err(B, n).\]
We also have 

\[ \left| \Vert \tilde{A} \Vert \Vert \tilde{B} \Vert - \Vert A\Vert\Vert B \Vert \right| \le \Vert  A \Vert \cdot \err(B,n) + \err(A, n) \cdot \Vert  B \Vert + \err(A, n) \err(B, n).  \]

Finally, combining the last two inequalities we have 

\begin{equation}
    \label{eqn:errC}
    \err(C, n) \le \mu(n) \mach \Vert {A} \Vert \Vert {B} \Vert +  (1+\mu(n) \mach)\left[ \Vert  A \Vert \cdot \err(B,n) + \err(A, n) \cdot \Vert  B \Vert + \err(A, n) \err(B, n) \right]
\end{equation}
Following \cite{demmel2007fast} define $\err(n)$ to be a bound for the maximum normwise error of the inverse of any $n \times n$ subblock of $T$ computed during the algorithm.

We also use the facts $\Vert T_{ii} \Vert \le \Vert T \Vert $ and $\Vert T_{ii}^{-1} \Vert \le \Vert T^{-1} \Vert$.

We now have 

    $\err(T_{ii}^{-1}, n/2) \le \err(n/2)$ 
    
     \begin{align*}\err(T_{11}^{-1} \cdot T_{12}, n/2) &\le \mu(n/2) \mach \Vert T_{11}^{-1} \Vert \Vert T_{12} \Vert + (1+ \mu(n/2) \mach) \err(T_{11}^{-1}, n/2) \Vert T_{12} \Vert \\
    &\le \mu(n/2) \mach \Vert T^{-1} \Vert \Vert T \Vert + (1 + \mu(n/2) \mach)\err(n/2) \Vert T \Vert \\
    &=: I_1
    \end{align*}
     \begin{align*}
        \err( (T_{11}^{-1} \cdot T_{12}) \cdot T_{22}^{-1}, n/2) &\le \mu(n/2)\mach \Vert T_{11}^{-1} \cdot T_{12} \Vert \cdot \Vert T_{22}^{-1} \Vert \\
        &\qquad + (1 + \mu(n/2)\mach) \big[ \err(T_{11}^{-1} \cdot T_{12}, n/2) \cdot \Vert T_{22}^{-1} \Vert + \Vert T_{11}^{-1} \cdot T_{12} \Vert \cdot \err(T_{22}^{-1}, n/2) \\
        &\qquad \qquad \qquad \qquad\qquad + \err(T_{11}^{-1} \cdot T_{12}, n/2) \err(T_{22}^{-1}, n/2) \big] \\
        &\le \mu(n/2) \mach \Vert T^{-1} \Vert \Vert T \Vert \Vert T^{-1} \Vert \\
        &\qquad + (1 + \mu(n/2)\mach) \big[ I_1 \Vert T^{-1} \Vert + \Vert T^{-1} \Vert \Vert T \Vert \err(n/2) + I_1 \err(n/2)\big] \\
        &=: I_2
        \end{align*}

\begin{align*}
    \err(T^{-1}, n) &\le \err(T_{11}^{-1}, n/2) + \err(T_{22}, n/2) + \err((T_{11}^{-1} T_{12}) T_{22}^{-1}, n/2) \\
    &\le 2\err(n/2) + I_2
\end{align*}

This finally yields the recurrence

\[ \err(n) \le (2 + 2(1+\mu(n/2)\mach)^2\kappa(T)) \err(n/2) + (1+\mu(n/2)\mach)^2 \kappa(T) \err(n/2)^2 + (1+\mu(n/2)\mach) \mu(n/2)\mach \kappa(T) \Vert T^{-1} \Vert.\]

(never mind, err is $<$ 1) \textcolor{red}{The $\err(n/2)^2$ on the right is a problem.  Its presence alone already means $\err(n)$ grows exponentially.  It does not appear in DDH07 because DDH07 discards the second-order term $\err(A)\err(B)$ in the matrix multiplication error. }
The stack trace of the term is as follows: It comes from $I_2$, which contains the term $I_1 \err(n/2)$, and inside $I_1$ there is another $\err(n/2)$.

Here's the simplest instance of a problem that reproduces the error in DDH07.  Suppose you have a problem for an $n \times n$ matrix $A$ that reduces to multiplying two $n/2 \times n/2$ matrix subproblems.  As a simple but valid example, suppose your problem is to raise a scalar $A = a$ to the power $n$, and the algorithm is repeated squaring (with error) $\log n$ times.  

By the DDH07 analysis, the error recurrence is roughly

\[\err(n) \le \mu(n) \mach \Vert A \Vert^2 + \Vert A \Vert \err(n/2),\]
yielding $\err(n) = O(\Vert A \Vert^{\log n} \mu(n) \mach)$.

But if you include the second-order term in the matrix multiplication error, you get
\[ \err(n) \le\mu(n) \mach \Vert A \Vert^2 + 2 \Vert A \Vert \err(n/2) + \err(n/2)^2,\]
and the solution of this is exponential.

==> Content/oldintro.tex <==

 We study the {\em approximate diagonalization} problem: given a square complex matrix $A\in\C^{n\times n}$ and parameter $\beta>0$, produce a diagonal $D$ and invertible $V$ such that
\begin{equation}\label{eqn:main} \|VDV^{-1}-A\|\le \beta\end{equation}
The diagonalization problem must necessarily be solved approximately since it is impossible to exactly compute eigenvalues in finite time, or to represent them on a computer. 

    
\begin{remark}[Forward vs. Backward Error] There are two reasonable notions of approximation for the diagonalization problem. Backward error, which is the notion in \eqref{eqn:main}, asks to find the exact solution of a nearby problem. This is the standard notion in numerical analysis and scientific computing, where the matrix is assumed to anyway be given up to some machine precision.  It is  the appropriate notion of approximation if one wants to use $VDV^{-1}$ as an approximate representation of $A$, or as a way to evaluate $f(A)=Vf(D)V^{-1}$ for analytic functions $f(\cdot)$; see \cite{davies2007approximate} for details.

A more stringent requirement is {\em forward error}: given a diagonalizable matrix $A\in \C^{n\times n}$ exactly in some form (perhaps as rationals), produce $V', D'$ such that $\|V-V'\|\le \beta$ and $\|D-D'\|\le \beta$ for $A=VDV^{-1}$. This notion is more suitable for applications in pure mathematics, where, e.g., the multiplicity of an eigenvalue has an important meaning. Work on forward error eigenvector computation is often parameterized in terms of the minimum gap between two eigenvalues. To appreciate the difficulty of this version of the problem, consider e.g. the examples of Parlett and Lu \cite[Chapter 2]{parlett1992minimum}: there are $n\times n$ {\em integer symmetric tridiagonal} matrices with entries bounded by $n$ which have two distinct eigenvalues with a gap of size $\exp(-cn)$. 

We will only consider the backward error version of the problem \eqref{eqn:main} in this paper.
\end{remark}
%\end{enumerate}
\subsection{Results} 
\begin{theorem} There is an algorithm $[V,D]=\EIG(A,\beta)$ which solves the approximate diagonalization problem
in $T_\EIG(n)=$\todo{} arithmetic operations on a floating point machine with precision $\u$=\todo{}. In particular, this implies that it computes such a $[V,D]$ in \todo{} bit operations.
\end{theorem}
To the best of our knowledge, there were only two rigorous bounds for solving the general eigenpair problem prior to this work.

\begin{enumerate}
    \item  Armentano et al. \cite{armentano2018stable} proved a bound of $O(n^9/\beta^2)$ arithmetic operations. The polynomial dependence on $\beta$ in their result arises from a smoothed analysis: they show that their algorithm essentially exactly solves the perturbed problem $A+\beta G$ in this much time on average, which can then be interpreted as a backward error bound as in \eqref{eqn:backwardeig} on the original problem $A$.  They informally argue numerical stability of their algorithm, which is a homotopy continuation method. Such an argument if made rigorous should imply a running time ot $O(n^9\polylog(n)/\beta^2)$.
    \item Cai \cite{cai1994computing} showed that the Jordan form of a rational $n\times n$ matrix with entries of bit length $b$ can be computed in $\poly(n,b,\log(1/\beta))$ time without specifiying the degree of the polynomial. Reading the proof reveals that the dependence is at least $\Omega(n^{11})$. This is a symbolic algorithm where arithmetic is carried out exactly and the key difficulty is to bound the bit complexity of the rationals which appear in the computation.
\end{enumerate}
Our algorithm is inspired by smoothed analysis idea of \cite{armentano2018stable}, and follows this route, but obtains logarithmic rather than polynomial dependence on the size of the perturbation.

In fact, our theorem is a black box reduction from the diagonalization problem to the more basic problems of matrix multiplication, inversion, and QR factorization. 
\begin{theorem}[Meta Theorem]

\end{theorem}Since matrix multiplication is required to even verify the output of such a computation, our running time dependence on $n$ is optimal up to polylogarithmic factors.

The key subroutine in our algorithm is a provably fast and stable way to compute the {\em sign function} of certain matrices. Recall that

The algorithm itself is not new, and has been studied in the numerical analysis community for at least thirty years. The 

\subsection{Related Work}
\subsubsection{Random Matrix Theory}
\subsubsection{Numerical Analysis}
Burgisser, Nakatsukasa, QR, Higham Sign, Bai-Demmel-Gu, DDH papers.
\subsubsection{Theoretical Computer Science}
Cai, Vempala, Ben-Or Eldar, Victor Pan
\subsection{Techniques}


==> Content/oldstuff.tex <==

\subsubsection{Log-stability}
As above $g(z)= \frac{1}{2}(z^{-1}+z)$. We will now show that we still have convergence when noise is added in every step. 

That is, let $\tilde{A}_0 = A_0 =A$, $A_{k+1} = A_k+A_k^{-1}$ and $\tilde{A}_{k+1} = (\tilde{A}_k+\tilde{A}_{k}^{-1})(1+ E_k)$. 

So, if we assume that the perturbation $E_k$ is coming from the error of the inversion algorithm from  \cite{demmel2007fast}, we can bound the norm of $\norm{E_k}$ as follows. By their result and by  definition of log-stability

$$\frac{\|\tilde{A}_{k+1}-g(\tilde{A}_k)\|}{\|g(\tilde{A}_k) \|} \leq O(\varepsilon) \kappa_g(\tilde{A}_k)^{c\log n} + O(\varepsilon^2).$$
Now note that $\tilde{A}_{k+1}- g(\tilde{A}_k) = g(\tilde{A}_k) E_k$, so
$$\frac{\|\tilde{A}_{k+1}-g(\tilde{A}_k)\|}{\|g(\tilde{A}_k) \|} = \frac{\|g(\tilde{A}_k)E_k \|}{\|g(\tilde{A}_k)\|} \geq \frac{\|E_k\|}{\|g(\tilde{A}_k)\| \|g(\tilde{A}_k)^{-1}\|}$$
and combining the above inequalities we get
$$\|E_k\| \leq O(\varepsilon) \|g(\tilde{A}_k)\| \|g(\tilde{A}_k)^{-1}\| \kappa_g(\tilde{A}_k)^{c\log n} + O(\varepsilon^2)\|g(\tilde{A}_k)\| \|g(\tilde{A}_k)^{-1}\|.$$
Now, using the bound $\|X\| \leq \rho(X) \kappa_V(X)$ we get that $$\|g(\tilde{A}_k))\| \leq \kappa_V(g(\tilde{A}_k)) \rho(g(\tilde{A}_k)) = \kappa_V(\tilde{A}_k)\rho(g(\tilde{A})_k)$$
and similarly

$$\|g(\tilde{A}_k)^{-1})\| \leq  \kappa_V(\tilde{A}_k)\rho(g(\tilde{A})_k^{-1}).$$

Now note that $$\kappa_g(\tilde{A}_k) = \|\tilde{A}_k\| \|\tilde{A}_k^{-1}\|\leq \kappa_V(\tilde{A}_k)^2 \rho(\tilde{A}_k) \rho(\tilde{A}_k^{-1})$$
all together yielding 
 $$\|E_k\| \leq O(\varepsilon) \kappa_V^{2(c\log n +1)}(\tilde{A}_k) \rho(\tilde{A}_k) \rho(\tilde{A}_k^{-1})\rho(g(\tilde{A}_k)) \rho(g(\tilde{A}_{k+1})^{-1})+ O(\varepsilon^2) \kappa_V^2(\tilde{A}_k) \rho(\tilde{A}_k) \rho(\tilde{A}_k^{-1})  $$
\bigskip

\begin{lemma}[In progress]
If  $$\frac{\|A_k -\tilde{A}_k\|}{ \|A_k\|}\leq  \varepsilon \exp(p(\log n))$$  for some polynomial $p(x)$, and $$\max\{\kappa_V(A_k) \rho(A_k), \kappa_V(\tilde{A}_k)\rho(\tilde{A}_k) \}  \leq \exp(c \log n)$$
Then something ``similar" happens for $k+1$, where ``similar" is something strong enough such that the number of iterations don't screw up things. 
\end{lemma}

\begin{proof} This is why I think this could work: 
$$
\frac{\|\tilde{A}_{k+1}-A_{k+1}\|}{\|{A_{k+1}}\|} \leq \frac{\|\tilde{A}_{k+1}-g(\tilde{A}_{k}) \|}{\|g(A_{k})\|} + \frac{\|g(\tilde{A}_k)-g(A_k)\|}{\|g(A_{k})\|} \leq \frac{\|g(\tilde{A}_k)\|}{\|g(A_k)\|} \|E_k\|+ \frac{\|\tilde{A}_k-A_k\|}{\|A_{k}\|} \kappa_g(A_k) 
$$
And note that all  quantities in the right hand side  are $\varepsilon \exp(polylog(n))$. 
\end{proof}


\section{Drafts}

Since I'm still very confused about how should we write some things I think it's not a bad idea to write here some of the technical steps, and once we have some understanding of the details decide how to present them. 

\subsection{Newton's method}

\subsubsection{Exact arithmetic}

Seems this has been rewritten over and over in different papers, so maybe is not necessary to include it in the final version of our paper. See for example \cite{roberts1980linear}. However, I didn't find any reference where the constants are explicit so I'll write the argument here.  


Let $g(z) = \frac{1}{2}(z+z^{-1})$ and let $g^k(z)$ denote $k$ applications of the function $g$ to $z$. 

\begin{lemma}[Convergence for scalars]
Let $z = \gamma + i \eta$ with $\gamma > 0$. Then 
$$|g^k(z)-1| \leq \frac{\omega^{2^{k-1}}}{1-\omega^{2^{k-1}}} ,$$
where $\omega = 1- \frac{4\gamma}{(1+\gamma)^2+\eta^2}$. 
\end{lemma}

\begin{proof}
Set $z_0 = z$ and $z_{k} = z_{k-1}$.  We have 
$$\frac{z_{k+1}-1}{z_{k+1}+1} = \frac{z_k+z_k^{-1}-2}{z_k+z_k^{-1}+2} = \frac{z_k^2-2z_k+1}{z_k+2z_k+1} = \left( \frac{z_k-1}{z_k+1} \right)^2 $$
and hence we have for every $k$ that
$$\frac{z_{k}-1}{z_{k}+1} = \left(\frac{z_0-1}{z_0+1} \right)^{2^k}.$$
Hence, if we denote $\varepsilon_k = \left( \frac{z_0-1}{z_0+1} \right)^k$, the above equation translates into 
$$z_k-1 = (z_k-1+2) \varepsilon_k \implies z_k-1 = \frac{2\varepsilon_k}{1-\varepsilon_k}\implies |z_k-1| \leq \frac{2 |\varepsilon_k|}{1-|\varepsilon_k|}.$$
Since $\varepsilon_k = \varepsilon_1^{2^k}$.  It remains to compute $|\varepsilon_1|$. Note that
$$\frac{|z_0-1|^2}{|z_0+1|^2} = \frac{(\gamma-1)^2+ \eta^2}{(\gamma+1)^2+ \eta^2} = 1 - \frac{4\gamma}{(1+\gamma)^2+ \eta^2}.$$
\end{proof}

The above result lifts to diagonalizable matrices trivially. 

\begin{corollary}[Convergence for diagonalizable matrices]
Let $A$ be a diagonalizable matrix with eigenvalues $\lambda_1, \dots, \lambda_n$. Denote $\lambda_j = \gamma_j+ i \eta_j$,  $\omega_j = 1- \frac{4|\gamma_j|}{(1+|\gamma_j|)^2+ \eta_j^2}$, and $\omega = \max_j \{ \omega_j\}$. Then 
$$\|g^k(A)-\mathrm{sign}(A)\| \leq \frac{\kappa_V(A) \omega^{2^{k-1}}}{1-\omega^{2^{k-1}}} $$
\end{corollary}


\begin{proof}
Since $A$ is diagonalizable we have $\sigma(f(A)) = f(\sigma(A)) $ for any  function $f$ for which $f(A)$ makes sense. By applying the previous lemma to every eigenvalue we get that 
$$\rho[g^k(A)-\mathrm{sign}(A)] \leq \frac{\omega^{2^{k-1}}}{1-\omega^{2^{k-1}}}.$$
And since  any diagonalizable $X$ we have $\|X\| \leq \kappa_V(X) \rho(X)$, and $g$ preserves the condition number of $A$, the result follows. 
\end{proof}

\subsubsection{Invariant circles}

Let $\mu(z) = \frac{z-1}{z+1}$ and $\mathcal{H}^+ =  \{ z \in \mathbb{C} : \mathrm{Re}(z) > 0\}$. Note that for every $z \in \overline{\mathcal{H}^+}$ we have $|\mu(z)| \in [0, 1]$. On the other hand for every $\alpa \in [0, 1]$ the locus
$$C_\alpha = \{ z \in \overline{\mathcal{H}^+}: |\mu(z)| = \alpha \}$$
is a circle with center in the real line. More precisely, $C_\alpha$ has the interval $[\frac{1-\alpha}{1+\alpha}, \frac{1+\alpha}{1-\alpha}]$ as a diameter. Hence, if 
$$D_\alpha = \{ z \in \overline{\mathcal{H}^+} : |\mu(z)| < \alpha \},$$
then $D_\alpha$ is the open disk  enclosed by $C_\alpha$. We know that
$$g(D_\alpha ) = D_{{\alpha^2}}.$$
Also note that for every $x, y \in \mathcal{H}^+$ we have 
$$|\mu(x)- \mu(y)| \left| \frac{(x-1)(y+1)-(y-1)(x+1)}{(x+1)(y+1)} \right| \leq 2|x-y|.$$
Which means that for every $ \varepsilon \in \mathbb{C}$ we have that
$$D_\alpha + \varepsilon \subset D_{\alpha+ 2 |\varepsilon|},$$
provided that $D_\alpha + \varepsilon$ is still contained in $\mathcal{H}^+$. 

For $\alpha$ near $0$, the circle $C_\alpha$ has radius $\Theta(\alpha)$ and for $\alpha$ near $1$, the distance from the circle to the imaginary axis is $\Theta(1-\alpha)$.  For now, in this section $\epsilon$ denotes a bound on the eigenvalue perturbation, which should come from the size of the matrix perturbation and $\kappa_V$.

\begin{lemma}
Suppose $1-\alpha_0 > \gamma$.   Fix $\epsilon, \delta > 0$, where $\epsilon < \gamma$ and $\delta > 2\epsilon^2$.  Recursively define $\alpha_k = (\alpha_{k-1} + \epsilon)^2$.  Then for $N = N(\epsilon, \gamma, \delta) = $, we have $\alpha_N < \delta$.
\end{lemma}
\begin{proof}
We have  $a_k = (a_{k-1}+\epsilon)^2 \le a_{k-1}^2(1 + \epsilon/\delta)^2$ as long as  $a_k > \delta$.  Thus $a_N \le a_0^{2^N} (1 + \epsilon/\delta)^{2(2^N-1)}.$ Thus, if $\gamma = 1/poly(n)$, and $\epsilon/\delta = 1/poly(n) << \gamma$, then after $c \log n$ iterations, $\alpha$ will dip below $\delta$--that is, all eigenvalues will be contained in a ball of radius $O(\delta)$ around their sign.
\end{proof}
